LEGO: Synergizing Expert GraphRAG and Expert Chain-of-Thought for Legal Reasoning

Large language models are increasingly applied to high-risk domains such as law, yet complex legal reasoning remains limited by two structural challenges. First, existing RAG and GraphRAG methods emphasize lexical or semantic similarity while overlooking normative relations among legal provisions. Second, vanilla Chain-of-Thought prompting may generate plausible rationales without enforcing the normative structure of legal reasoning. To deal with the bottleneck of pipelines in the legal reasoning domain, we propose LEGO, a dual-module framework that synergizes Legal Expert GraphRAG and expert Chain-of-thought for complex legal reasoning. ExpertGraphRAG uses an expert-annotated civil code graph encoding these normative relations with a greedy normative-coverage retrieval algorithm to dynamically extract instance-specific provision subgraphs, while ExpertCoT organizes the retrieved provisions and case facts into structured Provision-Fact-Conclusion reasoning. With a Qwen3-8B backbone, LEGO achieves 40.53% exact-match accuracy on LawExamQA_Civil, outperforming the evaluated RAG and CoT baselines and performing comparably to the evaluated larger models, while remaining robust on multi-hop questions. It also achieves the best results among the evaluated baselines on the open-ended benchmarks. Ablation studies confirm the individual and complementary contributions of both modules, demonstrating LEGO's effectiveness in improving LLMs' complex legal reasoning ability. Code and dataset can be found in the link: https://github.com/BLK-WHT/LEGO

==> latex/synergy_formalization.tex <==
% =====================================================================
%  synergy_formalization.tex
%
%  Synergy-gain formalization block, intended to sit at the START of
%  the Results and Discussion subsection (\S 5.4 in lego_paper.tex).
%
%  Provides two synergy metrics --- Weak Synergy Gain (WSG) and
%  Additive Synergy Gain (ASG) --- plus a summary table mapping the
%  notation to its meaning and the confirmation criterion. The
%  LEGO-specific instantiation feeds directly into Obs.\ 4 of the
%  Results and Discussion section.
%
%  USAGE
%  -----
%  In lego_paper.tex, immediately after
%
%      \subsection{Results and Discussion}
%      \label{sec:results_discussion}
%
%  insert
%
%      \input{synergy_formalization}
%
%  REQUIRED PACKAGES (already in lego_paper.tex):
%      amsmath, booktabs, multirow.
% =====================================================================


\ref{sec:appendix_synergy}.



==> lexgo_motivation_proposal.tex <==
% LEGO motivation proposal.
% This is a standalone draft. It has NOT been inserted into latex/lego_paper.tex.
% Suggested placement: replace the opening motivation paragraphs after
% \section{Introduction} and before the motivation figure.

The integration of LLMs into high-risk professional domains has accelerated rapidly, including law~\cite{chalkidis2022lexglue,NEURIPS2023_89e44582,blair2023can}. Yet these domains expose a structural gap in two widely used LLM augmentations. Retrieval-Augmented Generation (RAG) grounds generation in external evidence~\cite{NEURIPS2020_6b493230,yu2022survey}, while Chain-of-Thought (CoT) prompting externalises intermediate reasoning steps~\cite{wei2022chain}; recent surveys therefore frame RAG and reasoning as mutually reinforcing modules rather than isolated tricks~\cite{synergizingragreasoning2025}. In legal reasoning, however, simply placing RAG before CoT is not enough. A hard civil-law case is rarely solved by retrieving one statute or by writing a fluent rationale, but by chaining several provisions across multiple actors, legally relevant events, exceptions, prerequisites, and legal effects: the \textbf{subject\,$\times$\,event\,$\times$\,statute hop} triad.

The first bottleneck is retrieval. Standard RAG and many GraphRAG systems~\cite{microsoftgraphrag2024,survey_graphrag2025,linearrag2026,logicrag2026,hipporag2025,guo-etal-2025-lightrag} still rely heavily on lexical or embedding similarity, possibly over automatically induced graph neighbourhoods. Legal knowledge is often \emph{semantically sparse}: two provisions may look unrelated on the surface yet be tightly coupled by a prerequisite, exception, general--special, or legal-effect relation; conversely, two textually similar provisions may be doctrinal distractors because they belong to different constituent elements. Multi-hop QA work similarly shows that one-shot retrieve-then-read pipelines fail when what must be retrieved at step $t+1$ depends on what was established at step $t$~\cite{yang2018hotpotqa,trivedi2022musique,trivedi2023ircot}. For legal QA, the missing signal is therefore not merely ``more context'', but an explicit expert signal: human-curated links among statutes, concepts, elements, exceptions, priorities, and effects, together with a retrieval algorithm that can expose and score those links at inference time.

The second bottleneck is reasoning. Vanilla CoT and tree-style prompting can produce plausible intermediate text, but they do not guarantee that the model follows the normative order required by a professional domain~\cite{wei2022chain,yao2023tree}. In law, a reasoning trace can drift by skipping an exception, treating an unfulfilled prerequisite as satisfied, or affirming the consequent from a legal effect back to its condition. Retrieval-augmented reasoning helps only if the retrieved sources are authoritative and structurally relevant; otherwise, each generated step may amplify noise from the previous step, a risk also noted in faithfulness and robustness studies of RAG~\cite{brink2026,proberag2026}. Recent RAG--CoT systems interleave retrieval with reasoning~\cite{trivedi2023ircot}, revise thought steps with retrieved evidence~\cite{wang2024rat}, or use knowledge graphs to constrain CoT generation~\cite{li2025cotrag}; expert-guided medical QA further shows that domain attributes can constrain both retrieval and CoT in high-risk settings~\cite{ge2025expertems}. Legal reasoning requires an even more relational expert prior: \emph{legal relation $\rightarrow$ claim basis $\rightarrow$ constituent elements $\rightarrow$ exception/defence $\rightarrow$ legal effect}.

This motivates LEGO. We argue that robust multi-hop reasoning in knowledge-intensive, high-risk domains requires a complete expert pipeline: (i) experts pre-construct a domain graph according to the domain's own knowledge structure; (ii) a matched GraphRAG algorithm retrieves, expands, and ranks the graph so that expert links become explicit model input; and (iii) an expert CoT schema explains and applies those retrieved structures under domain-specific reasoning constraints. LEGO instantiates this recipe for civil-law QA by coupling an expert-curated Civil Code graph with statute-level graph retrieval and a dynamic Graph-of-Thought syllogistic prompt. The same design principle is domain-general: when experts can pre-encode the field's relational structure, RAG supplies trustworthy and structured evidence, while expert CoT turns that evidence into constrained multi-hop reasoning.

% Suggested BibTeX entries for citations introduced above.
% Add these to latex/lexgo.bib only if the motivation block is adopted.

@inproceedings{NEURIPS2020_6b493230,
 author = {Lewis, Patrick and Perez, Ethan and Piktus, Aleksandra and Petroni, Fabio and Karpukhin, Vladimir and Goyal, Naman and K\"{u}ttler, Heinrich and Lewis, Mike and Yih, Wen-tau and Rockt\"{a}schel, Tim and Riedel, Sebastian and Kiela, Douwe},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Larochelle and M. Ranzato and R. Hadsell and M.F. Balcan and H. Lin},
 pages = {9459--9474},
 publisher = {Curran Associates, Inc.},
 title = {Retrieval-Augmented Generation for Knowledge-Intensive NLP Tasks},
 url = {https://proceedings.neurips.cc/paper_files/paper/2020/file/6b493230205f780e1bc26945df7481e5-Paper.pdf},
 volume = {33},
 year = {2020}
}

@article{synergizingragreasoning2025,
    author    = {Yunfan Gao and Yun Xiong and Yijie Zhong and Yuxi Bi and Ming Xue and Haofen Wang},
    title     = {Synergizing {RAG} and Reasoning: A Systematic Review},
    journal   = {arXiv preprint arXiv:2504.15909},
    year      = {2025},
}

@inproceedings{trivedi2023ircot,
    author    = {Harsh Trivedi and Niranjan Balasubramanian and Tushar Khot and Ashish Sabharwal},
    title     = {Interleaving Retrieval with Chain-of-Thought Reasoning for Knowledge-Intensive Multi-Step Questions},
    booktitle = {Proceedings of the 61st Annual Meeting of the Association for Computational Linguistics},
    year      = {2023},
}

@article{wang2024rat,
    author    = {Zihao Wang and Anji Liu and Haowei Lin and Jiaqi Li and Xiaojian Ma and Yitao Liang},
    title     = {{RAT}: Retrieval Augmented Thoughts Elicit Context-Aware Reasoning in Long-Horizon Generation},
    journal   = {arXiv preprint arXiv:2403.05313},
    year      = {2024},
}

@inproceedings{li2025cotrag,
    author    = {Feiyang Li and Peng Fang and Zhan Shi and Arijit Khan and Fang Wang and Weihao Wang and {Zhangxin-hw} and Yongjian Cui},
    title     = {{CoT-RAG}: Integrating Chain of Thought and Retrieval-Augmented Generation to Enhance Reasoning in Large Language Models},
    booktitle = {Findings of the Association for Computational Linguistics: EMNLP 2025},
    year      = {2025},
    pages     = {3119--3171},
    publisher = {Association for Computational Linguistics},
    doi       = {10.18653/v1/2025.findings-emnlp.168},
}

@inproceedings{ge2025expertems,
    title     = {Expert-Guided Prompting and Retrieval-Augmented Generation for Emergency Medical Service Question Answering},
    author    = {Ge, Xueren and Murtaza, Sahil and Cortez, Anthony and Alemzadeh, Homa},
    booktitle = {Proceedings of the AAAI Conference on Artificial Intelligence},
    year      = {2026},
    note      = {Available as arXiv preprint arXiv:2511.10900},
    doi       = {10.48550/arXiv.2511.10900},
    url       = {http://arxiv.org/abs/2511.10900},
}

